Fine-Grained Egocentric Hand-Object Segmentation: Dataset, Model, and Applications

Egocentric videos offer fine-grained information for high-fidelity modeling of human behaviors. Hands and interacting objects are one crucial aspect of understanding a viewer's behaviors and intentions. We provide a labeled dataset consisting of 11,243 egocentric images with per-pixel segmentation labels of hands and objects being interacted with during a diverse array of daily activities. Our dataset is the first to label detailed hand-object contact boundaries. We introduce a context-aware compositional data augmentation technique to adapt to out-of-distribution YouTube egocentric video. We show that our robust hand-object segmentation model and dataset can serve as a foundational tool to boost or enable several downstream vision applications, including hand state classification, video activity recognition, 3D mesh reconstruction of hand-object interactions, and video inpainting of hand-object foregrounds in egocentric videos. Dataset and code are available at: https://github.com/owenzlz/EgoHOS

==> figs/data_sources.tex <==
\begin{figure*}[h]
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=0.8in 2.7in 0.8in 0in, clip,width=\textwidth]{data_sources.pdf}
    % \vspace{-20 pt}
    \caption{Extracted exemplar frames from multiple different sources of datasets. }
    \label{fig:hand_object_annotations}
    % \vspace{-10 pt}
\end{figure*}





==> figs/hand_object_annotations.tex <==
\begin{figure*}[h]
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=0.1in 5.1in 0.1in 0in, clip,width=\textwidth]{hand_object_annotations.pdf}
    % \vspace{-20 pt}
    \caption{A few example for hand and interacting object segmentation annotations. }
    \label{fig:hand_object_annotations}
    % \vspace{-10 pt}
\end{figure*}



